Red but not dead : Unveiling the Star-forming Far-infrared Spectral Energy Distribution of SpARCS Brightest Cluster Galaxies at 0 < z < 1.8

We present the results of a Spitzer/Herschel infrared photometric analysis of the largest (716) and highest-redshift (z=1.8) sample of Brightest Cluster Galaxies (BCGs), those from the Spitzer Adaptation of the Red-Sequence Cluster Survey (SpARCS). Given the tension that exists between model predictions and recent observations of BCGs at z<2, we aim to uncover the dominant physical mechanism(s) guiding the stellar-mass buildup of this special class of galaxies, the most massive in the Universe uniquely residing at the centres of galaxy clusters. Through a comparison of their stacked, broadband, infrared spectral energy distributions (SEDs) to a variety of SED model templates in the literature, we identify the major sources of their infrared energy output, in multiple redshift bins between 0 < z < 1.8. We derive estimates of various BCG physical parameters from the stacked {\nu}L{\nu} SEDs, from which we infer a star-forming, as opposed to a 'red and dead' population of galaxies, producing tens to hundreds of solar masses per year down to z=0.5. This discovery challenges the accepted belief that BCGs should only passively evolve through a series of gas-poor, minor mergers since z~4 (De Lucia & Blaizot 2007), but agrees with the improved semi-analytic model of hierarchical structure formation of Tonini et al. (2012), which predicts star-forming BCGs throughout the epoch considered. We attribute the star formation inferred from the stacked infrared SEDs to both major and minor 'wet' (gas-rich) mergers, based on a lack of key signatures (to date) of the cluster cooling flows to which BCG star formation is typically attributed, as well as a number of observational and simulation-based studies that support this scenario.

==> float/README <==

  The float package
  =================

This package improves the interface for defining floating objects such
as figures and tables in LaTeX.  It adds the notion of a `float style'
that governs appearance of floats.  New kinds of floats may be defined
using a \newfloat command analogous to \newtheorem.  This style option
also incorporates the functionality of David Carlisle's style option
`here', giving floating environments a [H] option which means `PUT IT
HERE' (as opposed to the standard [h] option which means `You may put
it here if you like').

Run `float.ins' through LaTeX to produce float.sty from float.dtx.
Run `float.dtx' through LaTeX to produce the documentation.

This program can be redistributed and/or modified under the terms
of the LaTeX Project Public License distributed from CTAN archives
in the directory macros/latex/base/lppl.txt; either version 1 of
the License, or (at your option) any later version.

                                Anselm Lingnau <anselm@strathspey.org>


==> titlesec/CHANGES <==
Titlesec changes

History of v1.0
~~~~~~~~~~~~~~~
1998/02/25  Added nops option
1998/02/28  Added \@mkboth stuff in \setmarks
1998/03/01  Changed test in \ttl@secnum
1998/03/03  Corrected some \fil... commands
1998/03/03  Replaced the faulty \@hangfrom by new commands
1998/03/03  Some \def replaced by \newcommand
1998/03/04  .dtx/.ins scheme finally rejected. Useless
            for users, obtrusive for `readers' and proned
            to errors
1998/03/04  Tidied up documentation
1998/03/06  \wordsep renamed and documented
1998/03/06  Added dummy asignation in \ttl@chap.
1998/03/06  Removed \ttl@xsect and merged into \tl@sect
1998/03/06  Added \ProvidesPackage

History of v1.1
~~~~~~~~~~~~~~~~
1998/03/25  \chapter corrected, as well as the size options
1998/03/26  Added compact option
1998/03/26  Added flushleft, flushright and center options
1998/04/08  Changed all instances of \noindent by \parindent\z@
1998/04/14  Added \filinner, \filouter
1998/04/14  Added drop shape
1998/05/01  Added rightmargin shape (and margin renamed to
            leftmargin)
1998/05/03  Added \setheadindent

History of v1.2 (unreleased)
~~~~~~~~~~~~~~~~~~~~~~~~~~~~~

1998/06/01  Compatibility with AMS classes
1998/06/08  On-demand loading of shapes
1998/06/11  Frame shape. Some \fil... command
            modified to work in the label of this
            chapter shape.
1998/07/03  Bottomtitle option (at last...)
1998/07/14  ...margin styles bug fixed using a method
            similar to bottomtitle.
1998/07/29  \titleline

====================

History of v2.0
~~~~~~~~~~~~~~~~

1998/08/05 to
1998/08/29  Fully reimplemented

History of v2.1
~~~~~~~~~~~~~~~~
1999/01/05  We define in this file the three basic shapes.
            Additional ones remain defined in external files.
            Unified the shapes for sections and chapters.
1999/01/05  \ttl@shape merged into \ttl@format@iii.
1999/01/05  \titlerule
1999/01/07  \ttl@defkeys splitted from \ttl@keys
1999/01/10  Added the \part stuff, including a definition of \@openright
1999/01/11  Removed unnecessary \ttl@numsecfalse in \ttl@sect@i.
1999/01/14  Optimized \titlerule
1999/01/27  Changed \titleline to correct the spacing at the
            top page and to fix a bug which changed the mode
            to horizontal, thus introducing unwanted space
            (\makebox -> \@makebox).
1999/02/02  \ttl@secnum renamed to \ttl@write and introduced the
            \ttl@savewrite mechanism to sincronize the toc/marks
            with the title in case there is a \newpage in <after>.
1999/02/03  wrap shape
1999/02/03  Added a \kern\z@ for not to avoid hyphenation
            of the last word. Not strictly necessary, but
            it is more LaTeX-like.
1999/02/05  \partmark defined (and in \setmarks, too).
1999/02/08  \ttl@row@i simplified.
1999/02/08  \ttl@savefn mechanism.
1999/02/10  Removed extra \leavevmode in display
1999/02/13  Now \titleline doesn't add the width. It's set.
1999/02/17  The part mark is catched, even if unused.
1999/02/17  old/newparttoc added.
1999/02/18  Changed many TeX assignments to the LaTeX
            counterpart.
1999/02/19  Introduced \ttl@startargs.

History of v2.1.1
~~~~~~~~~~~~~~~~~
1999/08/04  Moved misplaced lines in \ttl@makeboth

History of v2.2 (unreleased)
~~~~~~~~~~~~~~~~~~~~~~~~~~~~
1999/11/03  We load titleps if pagestyles are required, but
            some old definitions are restored.
1999/11/06  Improved outermarks test in \ttl@sect@i. Formerly
            the section number could be printed if a page ended
            with an unnumebered section followed by a numbered one.
1999/11/06  \ttl@startargs now adds (and passes) automatically the
            section name. Involved macros modified accordingly.
1999/11/06  Replaced explicit part names by the parameter in 
            \ttl@part@i. The same for chapter.
1999/11/21  \ttl@try's are not given explicitly, but built by
            \ttl@setkeys. Intruduced the \ttl@key@... and
            \ttl@extra@... commands.
1999/11/23  Minor problems with keys fixed.
1999/12/10  Added the nobottomtitles* option and \ttl@addstretch.
2000/01/07  First steps towards the calcwidth feature (basic code). 
2000/01/08  (Continued.) \titleline* for rules of width \titlewidth.
            Option calcwidth implemented.
2000/01/12  Finished with changes in wrap.tss (no longer
            "experimental" :-) ) 

History of v2.3
~~~~~~~~~~~~~~~
2000/01/19  All keys are grouped in a single file tttkeys. Removed
            page.tsk and deleted the corresponding code in the sty.
2000/01/19  Classes begun.
2000/01/19  The level numbers are stored in \ttll@ macros, and not
            passed as arguments.
2000/01/21  Introduced the new mark scheme. It's mostly compatible
            with the old one, but a compatibility mode seems
            imposible (it was introduced in a preliminary test
            but eventually removed).
2000/01/23  loadonly package option.
2000/02/01  Classes finished. Many things had to be rewritten.
2000/02/02  Made partially compatible with hyperref (dvips).
2000/02/08  \ttl@savewrite moved from shapes to classes. But
            explicit page breaks expand it, too, to avoid wrong
            toc entries.
2000/02/18  A new box named \ttl@box stores the title in runin
            leftmargin etc shapes, to increase reliability.
            
(2.3.1 -- 2.3.3  No changes on this file)
            
History of v2.3.4
~~~~~~~~~~~~~~~~~        
2000/05/12  nonindentfirst redefine \titlespacing instead of
            \@afterindent... so that they don't interfere with
            the first entry in tocs.
2000/05/17  The marks in \ttl@select are protected to prevent
            endless loop if the title is expanded, say, by 
            \MakeUppercase.
     
History of v2.3.5
~~~~~~~~~~~~~~~~~        
2000/05/21  Restores missing test for secnumdepth in \ttl@mkchap,
            and instead of setting \ttl@toclevel in ttlps now is
            done in \secdef. Except inside the macros, \ttl@toclevel
            is false, so that an explicit \...mark works. 
2000/06/04  \partmark defined with \providecommand
2000/06/14  A patch mechanism added, for small bug fixes.

History of v2.4
~~~~~~~~~~~~~~~~
2001/01/18  Minor changes in code. Essentialy an incremental
            update.
2001/01/22  \titleformat has a new "easy" starred variant.

History of v2.5
~~~~~~~~~~~~~~~
2002/01/02  New macros for \ttl@assign. Now * length allow
            non integer values.
2002/03/22  Added \ttl@calc and \ttl@calcneg to make titlesec
            calc-savvy.
         -  Merged bug fixes of .new into this file.
         -  Bugs in frame fixed -- gap in lines, misplaced
            label, wrong margins (sometimes),
         -  \leftskip, \rightskip and \linewidth (re)set in
            margin shapes.
         -  Removed obsolete flush... options.
         -  indentafter and noindentafter, new names for
            indentfirst and nonindentfirst.
         -  A new level (\titleclass) without its "location"
            now raises a meaningful error.
         -  Bug in top-level \titleclass fixed.
2002/03/23  Tests for undefined and unformatted sectioning levels,
            and horizontal material in <format>.
         -  Missing \if@openright inside \if@twoside in
            page class added.
         -  Removed extra (but inoffensive) \expandafter
            in \ttl@class@iii.
2002/03/27  Added \titlewidthfirst and ...last
         -  "Not definable" gives a  more meaningful message in
            the context of the package.

History of v.2.6
~~~~~~~~~~~~~~~~
2004/08/30  Corrected typo in margin \hsiz -> \hsize.
2004/10/17  Added a couple of missing \noexpand's in drop.
2004/12/01  Removed the error about the mode in block because this
            style is general purpose.
2005/01/16  Missing braces around #2 in the last else part of
            \ttl@headinline added
         -  Replaced explicit \makeatother's by a saved value as
            the macros can be used in a class/package file.
2005/01/18  newlinetospace mechanism
         -  // does not break pages; option pageatnewline to
            restore the LaTeX behaviour.
2005/01/19  \...break in top shape. 
         -  Renumbered several scratch registers to follow the
            TeXbook (p. 346), with \ttl@box in a few cases. In
            wrap \titlewidthfirst and \titlewidthlast made global.
         -  Float heads and foots have now a further argument for
            additional stuff (eg, to remove rules). Option is now
            psfloats while floatps enters in compatibility mode.
         -  \ttl@savetitle in all classes. Option toctitles.
2005/01/21  Changed pageatnewline to make it compatible with
            titletoc, with \ttl@changecentercr.
2005/01/22  \...tolist in top class.

History of v.2.7
~~~~~~~~~~~~~~~~
2007-03-27  Added the `explicit' option.
         -  Added \titlepagestyle.
2007-03-29  Fixed wrong number for chapter in log
         -  Patch file named .270 instead of .new
2007-05-09  Added <after> to leftmargin, so that you can add stuff
            at the beginning of the paragraph, eg, the sec number.
2007-07-07  Removed the patch mechanism.
2007-08-07  `explicit' improved.

History of v.2.8
~~~~~~~~~~~~~~~~
2007-08-12  \titlepagestyle already used by KOMA-Script. Renamed
            to \assignpagestyle.

History of v.2.9
~~~~~~~~~~~~~~~~ 
2010-05-04  Add \nobreak in \ttl@addcontentsline, to prevent the title
            going to footnotes (!) in runin style in some (rare) cases.
2010-05-06  Option uppercase (and \ttl@case).
2011-02-25  \iftitlemeasuring test
2011-07-14  Fixed \assignpagestyle
2011-07-15  Introduced the \scantokens mechanism to make sure section
            names are 'letters' and not 'others'
2011-07-18  Removed \if@nobreak test in wrap/drop, which added a line
            to the title after another section (why?)

History of v.2.9.1
~~~~~~~~~~~~~~~~~~
2011-08-28  Removed a spurious > in wrap.tss

History of v.2.9.2
~~~~~~~~~~~~~~~~~~
2011-11-11  Fixed a typo in ttlps.def (\MessageBreag)

History of v.2.10.0
~~~~~~~~~~~~~~~~~~~~

2011-12-15  Split titlesp

History of v.2.10.1
~~~~~~~~~~~~~~~~~~~~

2015-02-27  Fix: An explict \newpage in 'after' wrote the toc entry twice
2015-03-09  Fix (partial): A list containing just a sectioning command
            raised an error

History of v.2.10.2
~~~~~~~~~~~~~~~~~~~~

2015-03-21  Fix: With 2.10.1 labels vanished in hang shape (due to a
            misplaced \noindent)

History of titleps v.1.1.1
~~~~~~~~~~~~~~~~~~~~~~~~~~
2016-03-15  New macro \setmarkboth for compatibility



==> titlesec/README <==
This directory holds 3 packages for sectioning titles -- when used as
such (titlesec), in headers and footers (titleps) and in tables of
contents (titletoc).  They can be used separately, but you will get
most of them when used together.

Titlesec
~~~~~~~~
Sectioning titles, including margin and `wrap' titles, different
format in odd and even pages, rules above and below the title, 
adding new sectioning levels, measuring the width of the title, etc.

Titletoc
~~~~~~~~
TOC entries, with the possibility of changing the format in the middle
of a document, grouping the entries in a single paragraph, pretty
free-forms entries, partial tocs, etc.  It's described in titlesec.pdf
(or .tex).

Titleps
~~~~~~~
Page styles with working top marks, access to top, first and bot marks
in a single header/footer, rules, headers/footers for specific floats
(kinda \thispagestyle), multiple sets of marks, etc.  An one-stage
mechanims is used, without intermediate \leftmark's or \rightmark's.

What's new (2.9. 2.10)
~~~~~~~~~~~~~~~~

- Fixed \assignpagestyle, which did not work except in a 
few cases.
- Fixed an incompatibility with hyperref (wrong appendix 
name).
- Added \iftitlemeasuring
- Added package option uppercase
- Fixed a bug when reckoning the number of lines in wrap/drop.

2.9.1: Fixed a typo (a spurious > in wrap.tss).
2.9.2: Fixed another typo (\MessageBreag in ttlps.def)
2.10.0: New features in titleps also available in titlesec

Installation
~~~~~~~~~~~~
No .ins/.dtx preinstalation is required.  Move the files to a place 
where LaTeX can find them and typeset titlesec.tex.  All of files in 
this directory are necessary for titlesec.sty to work, except the 
manual titlesec.tex (and this 'readme' file). The manual requires
titlesec.sty and titletoc.sty, and hence all the .tss and .def 
files as well.

Formerly there were files with extension .new (titlesec.new and
titletoc.new) used to patch the packages, but if present should be
removed (they will be ignored, however).

Web site, manual in PDF format and info
~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~
Further details are available on

   http://www.texnia.com/titlesec.html

Contact
~~~~~~~
Please, for suggestions, bug reports, etc., go to
More
   http://www.texnia.com/contact.html

Known problems
~~~~~~~~~~
Some language styles (for babel) add the indentation
after a section in a so radical way that titlesec (which
uses the internal LaTeX macros) cannot supress it again.
For example, spanish (fixed in version 5.0) and frenchb.

2016/03/21


